Beyond Positive History: Re-ranking with List-level Hybrid Feedback

As the last stage of recommender systems, re-ranking generates a re-ordered list that aligns with the user's preference. However, previous works generally focus on item-level positive feedback as history (e.g., only clicked items) and ignore that users provide positive or negative feedback on items in the entire list. This list-level hybrid feedback can reveal users' holistic preferences and reflect users' comparison behavior patterns manifesting within a list. Such patterns could predict user behaviors on candidate lists, thus aiding better re-ranking. Despite appealing benefits, extracting and integrating preferences and behavior patterns from list-level hybrid feedback into re-ranking multiple items remains challenging. To this end, we propose Re-ranking with List-level Hybrid Feedback (dubbed RELIFE). It captures user's preferences and behavior patterns with three modules: a Disentangled Interest Miner to disentangle the user's preferences into interests and disinterests, a Sequential Preference Mixer to learn users' entangled preferences considering the context of feedback, and a Comparison-aware Pattern Extractor to capture user's behavior patterns within each list. Moreover, for better integration of patterns, contrastive learning is adopted to align the behavior patterns of candidate and historical lists. Extensive experiments show that RELIFE significantly outperforms SOTA re-ranking baselines.

==> backup.tex <==
\section{Introduction}
Due to the computational limits 
 facing numerous users and items, multi-stage recommender systems (MRS) have become ubiquitous in today's online platforms, such as Google~\cite{seq2slate}, YouTube~\cite{wilhelm2018practical}, and Taobao~\cite{prm}. A typical MRS comprises three stages in general, \ie, recall, ranking, and re-ranking, with each stage narrowing down the relevant items with a more complex but more accurate model for the sake of low response
latency \cite{liu2022neural}. 
As the final stage of MRS, re-ranking emphasizes modeling user preference and the listwise context between candidate items in order to generate a re-ordered list that aligns with the user's preferences. The re-ranked list is directly presented to the user and impacts the user's experience and satisfaction, showcasing the crucial position of re-ranking in MRS. 

Recently, much attention has been paid to the re-ranking stage, evolving from early efforts that primarily model the listwise context of candidate sets~\cite{dlcm,prm,setrank,seq2slate,qian2022scope,irgpr} to those that emphasize the importance of user preferences and how the preferences interact with candidate items~\cite{li2022pear,xi2022multi,shi2023pier,ren2023slate}. Pioneering works such as DLCM~\cite{dlcm}, PRM~\cite{prm}, and IRGPR~\cite{irgpr} explore the use of RNNs, transformers, and GNNs to model the mutual influences between candidate items. Subsequent advancements, \eg, PEAR~\cite{li2022pear} employs transformers to model user history behaviors, while MIR~\cite{xi2022multi} meticulously designs SLAttention to capture the relationship between the candidate set and user historical behaviors, significantly improving recommendation accuracy through the incorporation of user historical behaviors. 
Although previous work has achieved considerable success, they often leverage only users' positive feedback (\ie, clicked items) to extract user preferences, ignoring negative feedback (\ie, non-clicked items) and the relationship between positive and negative feedback.  In this work, we highlight that negative feedback and the relationship between positive and negative feedback also play crucial roles in modeling user preferences for re-ranking due to the following reasons. \ljh{should be distinguished. are we talking about the necessity of negative feedback (point 1), or the challenge of introducing negative feedback (point 2,3)? }
\ljh{NO INTRODUCTION FIGURE 1? \cb{may need one, the three points are too abstract}}

\ljh{maybe we can make the three points align with the three key component of our model. emphasizing the design motivation}

\textit{First, negative feedback can provide significant insights into user disinterest.} It could illustrate items or attributes that the user is not interested in or even dislikes, which positive feedback cannot reveal. For instance, if a user consistently provides positive feedback on a variety of products from brand A but also consistently exhibits negative feedback towards a specific category\ljh{of A? can it be more detailed?}, it suggests that while the user may generally favor brand A, they have a specific aversion to that category of brand A. \cb{maybe we can use a figure to depict this toy example?} This nuance is lost when relying solely on positive feedback, potentially leading to the erroneous conclusion that the user enjoys all products from brand A. Thus, the incorporation of negative feedback can provide more comprehensive insights into user interest modeling\ljh{a case of fine-grained}.

\textit{Second, leveraging only positive feedback could introduce bias, and the interaction between positive and negative feedback offers a more holistic understanding of user preferences\ljh{behavior patterns? since the negative feedback is more likely to be biased.}.} \cb{the difference between points 1 and 2 is indistinguishable. The point 1 also seems because of the bias when the brand = low-priced items} For instance, a user's previous clicks are all about low-priced items, leading to the assumption that she/he prefers low-priced items. However, if the user's negative feedback also consists of low-priced items, it indicates that the user does not necessarily prefer low-priced items over high-priced ones, but rather that the system's recent recommendations have predominated by low-priced items. 
Considering both positive and negative feedback simultaneously can mitigate the potential biases introduced by positive feedback alone, thereby offering a more comprehensive understanding of user preferences.


\textit{Lastly, the user's positive and negative feedback is influenced not only by user interests but also by user behavior patterns, especially comparison behavior manifesting within a list.} Many studies have revealed that a user might choose to click on a certain item after comparing it with surrounding ones, meaning positive feedback is influenced by negative ones~\cite{zhang2021constructing,fu2023f}. For example, if a user is currently interested in dresses and the list contains only dresses, she might compare the images of these dresses and choose the one that best matches her preferences. However, if the list contains only one dress, the user is likely to click on it even if it is not her favorite, simply because the surrounding items do not match her desires. Therefore, it is essential to account for user comparison patterns when modeling user interests from history lists and re-ranking candidate lists, as these behavior patterns significantly impact recommendations.


To address the aforementioned issues, we incorporate user list-level historical behaviors, \eg, the positive and negative feedback within each historical list, into re-ranking, considering both the impact of positive and negative feedback as well as user behavior patterns. We propose a framework named \underline{Re}-ranking with \underline{Li}st-level Historical \underline{Fe}edback (dubbed \textbf{RELIFE}), which extracts user interest preferences from three levels: item-level interests, intra-list patterns, and cross-list preferences, integrating the influence of candidate items. \textit{First}, we utilize \textbf{Dual Interest-Miner}\ljh{do we have -?} (DIM) module to separately capture the influence of positive and negative feedback on candidate items, extracting item-level user interests related to the candidate item. \textit{Second}, we device a \textbf{Comparison-aware Pattern Extractor} (CPE) unit to obtain list-level user patterns, which considers comparative behaviors within each list and leverage contrastive learning to align the pattern of the candidate list with that of the historical lists. \textit{Lastly}, we develop a \textbf{Sequential Preference Mixer} (SPM) module to learn the user's global preference under the influence of both positive and negative feedback within\ljh{across} multiple lists, incorporating temporal and candidate information. Our contributions can be summarized as follows:
\begin{itemize}
    \item We emphasize the pivotal role of list-level historical feedback in the user preference modeling of re-ranking. To the best of our knowledge, this is the first work to consider both positive and negative historical feedback and their relationships in re-ranking, \cb{do we need this? 'extracting a more ...'} extracting a more comprehensive user preference.
    \item We characterize user interests at different levels, with a Dual-Interest Miner, a Comparison-aware Pattern Extractor, and a Sequential Preference Mixer to capture item-level interests, intra-list patterns, and cross-list preferences.\ljh{respectively}
    \item Extensive experiments on two datasets demonstrate that our method significantly outperforms state-of-the-art re-ranking algorithms.\ljh{maybe talk about negative feedback like and can better utilize xxx}
\end{itemize}








==> body.tex <==

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{imgs/diver_network_structure.pdf}
%     \caption{Overall network structure.}
%     \label{fig:overall_framework}
% \end{figure*}

% \section{Problem Formulation}
%  \wwadd{$x_v$, $\Delta(S)$}Given a set of users $\mathcal U=\{1,\ldots,n_u\}$, a set of items $\mathcal V=\{1,\ldots,n_v\}$, and an initial ranking list $R(u)\in \Pi_L(\mathcal V)$ of $L$ items for users $u\in \mathcal U$, our task is to re-rank $R(u)$ and generate a list of $K$ distinct items $S(u)$ that better satisfies users' preferences and needs, usually $K<L$.
 
%  The probability of the user $u$ is attracted by item $v_k\in S(u)$ is a combination of two terms: a relevance term and a diversity term. The relevance of an item, in our setting, depends on the current item as well as local contexts and influence by other items in the list. The diversity term is the diversity gain in topic coverage, weighted by users' diversified interests towards different topics.
%  \begin{align}
%      \bar a_u(v_k) = &\lambda \phi_u(v_k|S(u))\tag{relevance}\\
%      &+ (1-\lambda)\langle\theta^u, \Delta(v_k|\{v_1,\ldots, v_{k-1}\})\rangle,\tag{diversity}\\\label{eq:diver_attr}
%  \end{align}
 
%   where $\phi_u(v_k|S(u))$ is relevance score of item $v_k$ given the presence of other items in the initial lists, and $\Delta(v_k|\{v_1,\ldots, v_{k-1}\})=c(\{v_1,\ldots, v_{k-1}\}\cup \{v_k\})-c(\{v_1,\ldots, v_{k-1}\})$ is the topic coverage gain by item $v_k$ over the previous $k-1$ items,  $\theta^u=(\theta^u_1,\ldots,\theta^u_m)$ is the personalized topic preferences of a user $u$, which is a distribution over $m$ topics.
 
% \begin{algorithm}[H]
% \caption{\texttt{Diver}}
% \begin{algorithmic}[1]
% \REQUIRE $u,R(u),K,\lambda, \Delta$, $\hat e_u$, $\hat a_u$, $\hat{\theta}^u$
% \ENSURE $S$
% \STATE $S\leftarrow\emptyset$
% \WHILE{$|S|< K$} 
% \STATE $v^*\leftarrow\arg\max_{v\in R\setminus S}P(v|u)+\lambda\tau_u P(v,\bar S|u)$
% \STATE $R\leftarrow R\setminus \{v^*\}$
% \STATE $S\leftarrow S\cup\{v^*\}$
% \ENDWHILE
% \RETURN $S$
% \end{algorithmic} 
% \label{alg:main}
% \end{algorithm}


 
 \section{Proposed Model}
 \subsection{Attractiveness Estimation}
 \subsubsection{Relevance}
 \begin{equation}
     \phi_u(v_k|S(u)) = f_\Phi(x_{v_k}|\{x_{v_1},\ldots,x_{v_K}\}, x_u)
 \end{equation}
 \subsubsection{Personalized Topic Preferences}
 The model takes as input the user positively interacted items grouped by different topics, and outputs the topic preferences $\hat \theta^u$.
 
 \subsection{Termination Estimation}
 \begin{equation}
     \hat e_u = f_\Theta(x_{v_k}|\{x_{v_1},\ldots,x_{v_K}\}, x_u)
 \end{equation}
 
 \subsection{Re-ranking}
 \wwadd{Use the upper bound, Ranking under uncertainty} We select the re-ranked list that maximizes the probability that a user feels satisfied
 \begin{equation}\label{eq:diver_max}
     S(u) = {\arg\max}_{A\in\Pi_K(R(u))}f(A, \hat e_u, \hat a_u).
 \end{equation}
 It can be easily shown that the expected reward is maximized when the attractiveness the items are listed in the same decreasing order of the termination probability.

\subsection{Optimization}
We optimize the lower bound of the log-likelihood of the dependent click model, to push the model to score satisfying items higher than the negative ones,
% \begin{align*}
%     \mathcal L_{lower} =&\sum_{k=1}^K \Big(y_u(v_k)\log\left( \hat{a}_u(v_k)\right)\\
%     + &\left(1- y_u(v_k)\right)\log\left(1-\hat{a}_u(v_k)\right)\Big)\\
%     + &\sum_{k=1}^{K-1}y_u(v_k)\log e_u(k) + \log(1-e_u(k)),\\
% \end{align*}

\begin{align*}
    \mathcal L_{lower} =&\sum_{k=1}^K \Big(y_u(v_k)\log\left( \hat{a}_u(v_k)\right) + \left(1- y_u(v_k)\right)\log\left(1-\hat{a}_u(v_k)\right)\Big)\\
    + &\sum_{k=1}^{K-1}y_u(v_k)\log (1-e_u(k)) + \log(e_u(K)),\\
\end{align*}
\wwadd{this objective function does not work well, need revise}

\section{Theoretical Analysis}
\input{theorem}


\section{Experiments}
\begin{itemize}
    \item (RQ1) How does Diver perform as compared with the state-of-the-art reranking models in terms of utility and diversity?
    \item (RQ2) How well does Diver perform on different scenarios with various importance of diversity?
    \item (RQ3) How well does Diver perform on different initial ranking lists?
    \item (RQ4) How do different hyper-parameter settings (the dimension of hidden states, \wwadd{and others?}) influence the performance of Diver?
    \item (RQ5) How does each designed component (the user history behaviors, the aggregation function) influence the performance of Diver?
\end{itemize}

\subsection{Dataset}
\subsubsection{Taobao}
Taobao data is a dataset consisting of user behavior data retrieved from Taobao\footnote{\url{https://tianchi.aliyun.com/dataset/dataDetail?dataId=649}}, one of the biggest e-commerce platforms in China, with 987,994 users, 4,162,042 items, and 100,150,807 interactions. It contains user behaviors from November 25 to December 3, 2017. We select top 10,000 users with the highest number of interactions, whose data from first 2 days is used to learn personalized topic preferences. And their next 3 days (3-5 days) are selected as training set, and following 3 day(6-8 day) and the last day are validation set and test set, respectively.  We use Gaussian Mixture Models(GMMs) to compute $h_j(v)$, the probability of item $v$ covering topic $j$.

\subsubsection{MovieLens-20M\footnote{\url{https://grouplens.org/datasets/movielens/20m/}}}
This dataset describes free-text tagging activity and 5-star rating for movies from MovieLens\footnote{\url{https://movielens.org/}}, a movie recommendation service. It contains 20000263 ratings and 465564 tag applications across 27278 movies, created by 138493 users between January 09, 1995 and March 31, 2015. We only remain users with more than 200 interactions, then we random shuffle all the remaining records and divide the data set into user profile history, training set, validation set, and test set in the ratio of 2:3:4:1. Given all the movies in MovieLens-20M belong to 20 genres, we use the normalized multi-hot genre vector as the probability of item $v$ covering topic $j$,  $h_j(v)$.

\subsubsection{Huawei Data}
Our algorithms are evaluated on a proprietary dataset obtained from Huawei App store. We use \textit{Gaussian Mixture Models} (GMMs) to compute $h_j(v)$ the probability of item $v$ covering topic $j$. Huawei data has 17 different categories: number of topics $m=17$?

\subsection{Click Feedback}
 \subsubsection{Dependent Click Model}
The system displays an ordered list of $K$ items to the user. The user examines the items in the displayed order and clicks on the attracted items. After an item
is clicked, the user may either be satisfied and leave, or proceed to the next item. The user leaves if all $K$ items have been examined, regardless of whether the user has found any satisfactory item or not.

For each user, the model is parameterized by $K$ \textit{item-dependent attraction probabilities} $\bar w_u\in[0,1]^K$, and $K$ \textit{position-dependent termination probabilities} $\bar e_u\in[0,1]^K$. The user checks the list of items one by one from top to bottom. For each item $v_k$, the user is attracted with probability $\bar a_u(v_k)$. If the user is attracted by $v_k$, then she clicks it and examines the item. The user may be satisfied and leave, which happens with probability $\bar e_u(k)$. The user may also continues to check the next item (which happens with probability $1-\bar e_u(k)$). If all items have been checked and the user has not found any satisfactory item, then the user leaves, unsatisfied.

The probability that a user $u$ is satisfied with list is
\begin{equation}
    f(S, \bar e_u, \bar a_u)=1-\prod_{k=1}^K\left(1-\bar e_u(k)\bar a_u(v_k)\right).
\end{equation}

\subsubsection{Submodular Diverse Model}
Suppose items belongs to $m$ topics, then the topic coverage of a list $c(S)\in[0,1]^m$, is an $m$-dimensional vectors whose $j$-th entry is the coverage of topic $j\in \{1,\ldots,m\}$. We assume $c_j(S)$ is a monotone and submodular function in $S$ for any $j\in \{1,\ldots,m\}$:
\begin{align}
    \forall S\subseteq S' & \subseteq \mathcal V, v\in \mathcal V:  \nonumber\\
    & c_j(S\cup \{v\})\geq c_j(S) \tag{monotonicity}\\
    \text{and}\: & c_j(S\cup \{v\}) - c_j(S) \geq c_j(S'\cup \{v\}) - c_j(S'). \tag{submodularity}
\end{align}
For example, a commonly adopted diverse function is the probabilistic coverage function,
\begin{equation}
    c_j(S) = 1 - \prod_{v\in S}(1-h_j(v)),
\end{equation}
where $h_j(v)$ is the probability of item $v$ covering topic $j$, and $c_j(s)$ is the $j$-th entry of $c(S)$, describing the probability of at least one item the list $S$ covers topic $j$. Clearly, such a function is monotone and submodular in each entry of $c(S)$.

\subsection{Evaluation Metrics}
\wwadd{\begin{itemize}
    \item accuracy-based: ndcg, map, clicks
    \item diversity-based: lntra list similarity, probabilistic coverage diversity
    \item Dependent click models.
\end{itemize}}


\subsection{Baselines}
\begin{itemize}
    \item DLCM
    \item Seq2Slate
    \item PRM
    \item SetRank
    \item MMR (search result diversification re-ranking method)
    \item Xquad (search result diversification re-ranking method)
\end{itemize}

\subsection{Initial Rankers}
\begin{itemize}
    \item \wwadd{DIN}
    \item SVMRank
    \item LambdaMart
    \item Urank (other learning to rank methods)
\end{itemize}

\subsection{Overall Performance}
\wwadd{The utility-diversity tradeoff exists widely.}
\wwadd{Initial ranker is not diversified, focusing a certain popular topics.}

% \begin{table*}[]
% \footnotesize
% \begin{threeparttable}
% \begin{tabular}{cccccc|ccccc}
% \toprule
%               & ndcg@3          & utility@3       & ILS@3           & diversity@3         & satisfaction@3     & ndcg@5          & utility@5       & ILS@5           & diversity@5         & satisfaction@5      \\ \midrule
% initial ranker & 0.2281          & \textbf{0.1657} & 2.7011          & 2.42502314          & 0.07603935          & \textbf{0.3085} & \textbf{0.2691} & 2.2518          & 3.33045927         & \textbf{0.15295046} \\
% prm            & 0.2274          & 0.1632          & 2.7013          & 2.42542491          & 0.07627046          & 0.3076          & 0.2664          & 2.2501          & 3.3302738          & 0.15218162          \\
% diver          & \textbf{0.2284} & 0.165           & \textbf{2.6997} & \textbf{2.42567061} & \textbf{0.07651311} & 0.3084          & 0.266           & \textbf{2.2492} & \textbf{3.3328366} & 0.15114638               \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=0.5$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5 & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.6482 & 1.2334  & 3.0854 & 0.221 & 0.5623 & 1.8755  & 4.221 & 0.1661   \\
% SetRank   &   0.6208 & 1.4593  & 3.1789 & 0.2573 & 0.5564 & 2.1065  & 4.2927 & 0.1835   \\
% % Seq2Slate &  & & & & & & &   \\
% DLCM      &  0.7071 & 1.7284  & 3.2719 & 0.2975 & 0.6755 & 2.4087  & 4.349 & 0.2056  \\
% PRM       &  \textbf{0.7267 }& 1.7893  & 3.1774 & 0.3064 & 0.6992 & 2.4519  & 4.2834 & 0.2083  \\

% \midrule
% MMR       &  0.6713 & 1.1002  & 2.3698 & 0.1992 & 0.545 & 1.8017  & 3.7387 & 0.1616   \\
% DPP       & 0.652 & 1.2564  & \textbf{3.4495} & 0.2247 & 0.5789 & 1.8625  & \textbf{4.4414} & 0.1644   \\\midrule
% Diver & 0.7098 & \textbf{1.8260} & 3.2858 & \textbf{0.3121} & 0.6858 & \textbf{2.5277 }& 4.4167 & \textbf{0.2144} \\
% \bottomrule
% % Diver-seq2seq & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=0.5$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2432          & 0.4103          & 3.0849          & 0.2227          & 1.8912          & 0.5054          & 4.2208          & 0.1674          & 1.8412          & 0.4936          & 5.6425          & 0.3190          & 2.3379          & 0.5383          & 7.1999          & 0.2743          \\
SetRank        & 1.6935          & 0.4553          & 3.1826          & 0.2925          & 2.2972          & 0.5629          & 4.2621          & 0.1963          & 2.0630          & 0.5185          & 6.2412          & 0.3511          & 2.6291          & 0.5692          & 7.8875          & 0.3032          \\
DLCM           & 1.7284          & 0.4933          & 3.2719          & 0.2975          & 2.4087          & 0.6039          & 4.3490          & 0.2056          & 2.0960          & 0.5438          & 6.5144          & 0.3555          & 2.6540          & 0.5924          & 8.1239          & 0.3055          \\
PRM            & 1.7893          & 0.5041          & 3.1774          & 0.3064          & 2.4519          & 0.6134          & 4.2834          & 0.2083          & 2.0911          & 0.5267          & 6.2818          & 0.3550          & 2.6560          & 0.5775          & 7.8888          & 0.3057          \\
\textbf{Diver} & \textbf{1.8260} & \textbf{0.5065} & \textbf{3.2858} & \textbf{0.3121} & \textbf{2.5277} & \textbf{0.6206} & \textbf{4.4167} & \textbf{0.2144} & \textbf{2.1068} & \textbf{0.5490} & \textbf{6.5634} & \textbf{0.3570} & \textbf{2.6623} & \textbf{0.5975} & \textbf{8.1706} & \textbf{0.3063}  \\\midrule
MMR            & 1.2560          & 0.4100          & 3.2464          & 0.2247          & 1.8938          & 0.5048          & 4.2611          & 0.1674          & 1.8575          & 0.4857          & 5.8207          & 0.3214          & 2.3455          & 0.5280          & 7.3301          & 0.2750          \\
DPP            & 1.3326          & 0.4259          & \underline{4.1645}          & 0.2377          & 1.8732          & 0.5023          & \underline{4.5851}          & 0.1645          & 1.9458          & 0.5065          & 6.4568          & 0.3342          & 2.4378          & 0.5480          & \underline{8.3408}          & 0.2846          \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}


% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=0.9$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5  & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.5287 & 1.2594  & 3.0854 & 0.2246 & 0.3835 & 2.1672  & 4.221 & 0.1923 \\
% SetRank   &  0.5417 & 2.2346  & 3.1658 & 0.3707 & 0.4912 & 3.1768  & 4.2632 & 0.2621 \\
% % Seq2Slate &  & & & & & & &   \\
% DLCM      &  0.7251 & 2.5603  & 3.195 & 0.4106 & 0.7028 & 3.4622  & 4.2731 & 0.2797   \\
% PRM       &  0.7627 & 2.5927  & 3.1974 & 0.4144 & 0.7464 & 3.5072  & 4.2738 & 0.2826     \\
% \midrule
% MMR       & 0.5342 & 1.2273  & 2.4744 & 0.2194 & 0.3817 & 2.1325  & 3.4594 & 0.1897   \\
% DPP       & 0.5373 & 1.2226  & \textbf{3.4495} & 0.219 & 0.3902 & 2.1023  & \textbf{4.4414} & 0.1872  \\\midrule
% % Diver   & \textbf{0.7657} & \textbf{2.6760} & 3.1982 & \textbf{0.4253} & \textbf{0.7555} & \textbf{3.5881} & 4.2807 & \textbf{0.2876 }\\
% Diver & 0.7562 & \textbf{2.6357} & 3.2001 & \textbf{0.4203} & 0.7427 & \textbf{3.5691} & \textbf{4.2813} & \textbf{0.2869} \\
% % Diver &  & & & & & & &   \\
% \bottomrule
% % Diver-seq2seq  & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}

\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=0.9$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2698          & 0.3302          & 3.0845          & 0.2264          & 2.1849          & 0.4331          & 4.2207          & 0.1937          & 1.7972          & 0.4067          & 5.6412          & 0.3103          & 2.4889          & 0.4418          & 7.1997          & 0.2871          \\
SetRank        & 2.3785          & 0.6152          & 3.1870          & 0.3893          & 3.3416          & 0.7159          & 4.2706          & 0.2731          & 2.2401          & 0.4820          & 5.8967          & 0.3738          & 3.0700          & 0.5273          & 7.5221          & 0.3428          \\
DLCM           & 2.5603          & 0.6872          & 3.1950          & 0.4106          & 3.4622          & 0.7769          & 4.2731          & 0.2797          & 2.2393          & 0.4871          & 5.8975          & 0.3736          & 3.0700          & 0.5324          & 7.5226          & 0.3428          \\
PRM            & 2.5927          & 0.7001          & 3.1974          & 0.4144          & 3.5072          & 0.7915          & 4.2738          & 0.2826          & 2.2428          & 0.4874          & 5.8957          & 0.3741          & 3.0735          & 0.5325          & 7.5191          & 0.3431          \\
\textbf{Diver} & \textbf{2.6357} & \textbf{0.7090} & \textbf{3.2001} & \textbf{0.4203} & \textbf{3.5691} & \textbf{0.8022} & \textbf{4.2813} & \textbf{0.2869} & \textbf{2.2437} & \textbf{0.4881} & \textbf{5.8995} & \textbf{0.3742} & \textbf{3.0740} & \textbf{0.5329} & \textbf{7.5254} & \textbf{0.3431} \\ \midrule
MMR            & 1.2636          & 0.3264          & 3.2439          & 0.2256          & 2.1824          & 0.4302          & 4.2708          & 0.1937          & 1.8005          & 0.4060          & 5.7282          & 0.3108          & 2.4905          & 0.4415          & 7.2514          & 0.2873          \\
DPP            & 1.2109          & 0.3188          & \underline{4.1641}          & 0.2174          & 2.0838          & 0.4164          & \underline{4.5847}          & 0.1858          & 1.8077          & 0.4052          & \underline{6.4558}          & 0.3119          & 2.4959          & 0.4406          & \underline{8.3398}          & 0.2879          \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

% \begin{table*}[]
% \centering
% \caption{Overall Performance. $\lambda=1$}
% \begin{threeparttable}
% \begin{tabular}{lllll|llll}
% \toprule
%           & MRR@5 & utility@5  & div@5 & satis@5 & MRR@10 & utility@10  & div@10 & satis@10 \\\midrule
% Init      &  0.5292 & 1.2660  & 3.0854 & 0.2256 & 0.3692 & 2.2402  & 4.221 & 0.1987 \\
% % Seq2Slate &   0.5288 & 1.2762  & 3.0848 & 0.2273 & 0.3693 & 2.2578  & 4.2206 & 0.2002   \\
% SetRank   &   0.5731 & 2.4516  & 3.1898 & 0.3994 & 0.5116 & 3.5506  & 4.2723 & 0.2884  \\
% DLCM      &   0.7509 & 2.7410  & 3.1961 & 0.4327 & 0.731 & 3.7163  & 4.2738 & 0.2966      \\
% PRM       &   \textbf{0.7995} & 2.7718  & 3.1944 & 0.4355 & \textbf{0.7891} & 3.7553  & 4.278 & 0.2993   \\
% \midrule
% MMR       & 0.5292 & 1.2660  & 3.0854 & 0.2256 & 0.3692 & 2.2402  & 4.2210 & 0.1987 \\
% DPP       & 0.5393 & 1.2142  & \textbf{3.4495} & 0.2177 & 0.3747 & 2.1623  & \textbf{4.4414} & 0.1928  \\\midrule
% Diver     & 0.7745 & \textbf{2.8400} & 3.1991 & \textbf{0.4449} & 0.7672 & \textbf{3.8464} & 4.2790 & \textbf{0.3050} \\
% % Diver &  & & & & & & &   \\
% \bottomrule
% % Diver-seq2seq  & & & & & & & & & & \\\bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*}


\begin{table*}[]
\centering
\scriptsize
\caption{Overall Performance. $\lambda=1.0$}
\begin{threeparttable}
\begin{tabular}{ccccc|cccc|cccc|cccc}
\toprule
               & \multicolumn{8}{c|}{Taobao}                                                                                                                    & \multicolumn{8}{c}{MovieLens-20M}                                                                                                             \\\cmidrule{2-17}
               & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        & util@5          & ndcg@5          & div@5           & satis@5         & util@10         & ndcg@10         & div@10          & satis@10        \\\midrule
Init           & 1.2761          & 0.3163          & 3.0845          & 0.2273          & 2.2578          & 0.4198          & 4.2204          & 0.2002          & 1.7862                                 & 0.3897                                 & 5.6412                                 & 0.3085                                 & 2.5265                                 & 0.4244                                 & 7.1992                                 & 0.2905                                 \\
SetRank        & 2.5298          & 0.6449          & 3.1922          & 0.4100          & 3.6154          & 0.7465          & 4.2759          & 0.2925          & 2.2823                                 & 0.4989                                 & 5.8110                                 & 0.3793                                 & 3.2359                                 & 0.5432                                 & 7.5369                                 & 0.3505                                 \\
DLCM           & 2.7410          & 0.7375          & 3.1961          & 0.4327          & 3.7163          & 0.8222          & 4.2738          & 0.2966          & 2.2857                                 & 0.5006                                 & 5.7986                                 & 0.3797                                 & 3.3456                                 & 0.5543                                 & 7.6914                                 & 0.3478                                 \\
PRM            & 2.7718          & 0.7517          & 3.1944          & 0.4355          & 3.7553          & 0.8378          & 4.2780          & 0.2993          & 2.2853                                 & 0.5008                                 & 5.8059                                 & 0.3797                                 & 3.1791                                 & 0.5417                                 & 7.4360                                 & 0.3524                                 \\
\textbf{Diver} & \textbf{2.8400} & \textbf{0.7639} & \textbf{3.1991} & \textbf{0.4449} & \textbf{3.8464} & \textbf{0.8511} & \textbf{4.2790} & \textbf{0.3050} & {\color[HTML]{7B7F83} \textbf{2.2854}} & {\color[HTML]{7B7F83} \textbf{0.5018}} & {\color[HTML]{7B7F83} \textbf{5.8081}} & {\color[HTML]{7B7F83} \textbf{0.3797}} & {\color[HTML]{7B7F83} \textbf{3.2894}} & {\color[HTML]{7B7F83} \textbf{0.5483}} & {\color[HTML]{7B7F83} \textbf{7.6129}} & {\color[HTML]{7B7F83} \textbf{0.3492}} \\ \midrule
MMR            & 1.2635          & 0.3127          & 3.2440          & 0.2256          & 2.2521          & 0.4172          & 4.2708          & 0.2000          & 1.7862                                 & 0.3902                                 & 5.6414                                 & 0.3085                                 & 2.5266                                 & 0.4248                                 & 7.1996                                 & 0.2905                                 \\
DPP            & 1.1792          & 0.2990          & \underline{4.1639}          & 0.2121          & 2.1347          & 0.4022          & \underline{4.5848}          & 0.1909          & 1.7733                                 & 0.3890                                 & \underline{6.4559}                                 & 0.3067                                 & 2.5109                                 & 0.4228                                 & \underline{8.3403}                                 & 0.2890                                 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

\begin{table*}[]
\centering
\small
\caption{Huawei App Store}
\begin{threeparttable}
\begin{tabular}{ccccccc}
\toprule
               & revenue@3                     & div@3                         & revenue@5                     & div@5                         & revenue@10                    & div@10                        \\\midrule
Init           & 1.7720                        & 0.1075                        & 2.4445                        & 0.1537                        & 3.4300                        & 0.2325                        \\
SetRank        & {\color[HTML]{A5A5A5} 1.6960} & {\color[HTML]{A5A5A5} 0.1071} & {\color[HTML]{A5A5A5} 2.3081} & {\color[HTML]{A5A5A5} 0.1519} & {\color[HTML]{A5A5A5} 3.2902} & {\color[HTML]{A5A5A5} 0.2286} \\
DLCM           & 1.8527                        & 0.1079                        & 2.5292                        & 0.1560                        & 3.5263                        & 0.2381                        \\
PRM            & 1.8708                        & 0.1082                        & 2.5382                        & 0.1556                        & 3.5025                        & 0.2356                        \\
\textbf{Diver} & \textbf{1.9075}               & \textbf{0.1096}               & \textbf{2.6228}               & \textbf{0.1579}               & \textbf{3.5625}               & \textbf{0.2386}               \\\midrule
MMR            & 1.3960                        & 0.1066                        & 2.1156                        & 0.1476                        & 3.2371                        & 0.2260                        \\
DPP            & 1.3686                        & \underline{0.1282}                        & 2.0921                        & \underline{0.2008}                        & 3.2310                        & \underline{0.2905}                        \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}


\begin{figure}[t] %hbt
	\vspace{-0pt}
	\centering
	\includegraphics[width=0.235\textwidth]{imgs/case_dive_hist.pdf}
	\includegraphics[width=0.235\textwidth]{imgs/case_dive_rerank.pdf}
	\vspace{-18pt}
	\caption{The distributions of items for a users with diverse interests. }
	\label{fig:sample}
	\vspace{-10pt}
\end{figure}

\begin{figure}[t] %hbt
	\vspace{-0pt}
	\centering
	\includegraphics[width=0.235\textwidth]{imgs/case_homo_hist.pdf}
	\includegraphics[width=0.235\textwidth]{imgs/case_homo_rerank.pdf}
	\vspace{-18pt}
	\caption{The distributions of items for a users with single interest. }
	\label{fig:sample}
	\vspace{-10pt}
\end{figure}

 \section{Literature Review}
 \subsection{Reranking for Recommender Systems}
 Several existing works have demonstrated the effectiveness of re-ranking by modeling item mutual influences and interactions in the initial ranking lists \cite{dlcm,prm,setrank,feng2021revisit}.
For example, Ai \etal \cite{dlcm} use a recurrent neural network to sequentially encode the top-ranked items with their feature vectors, and learn a local context model to re-rank the top results. Similarly, Zhuang \etal \cite{zhuang2018globally} design a recurrent neural network with an attention mechanism to capture long-distance influences between items.

Inspired by the Transformer architecture \cite{vaswani2017attention} used in machine translation, Pei \etal \cite{prm} propose to use the Transformer to model the mutual influences between items. The Transformer structure uses the self-attention mechanism where the relationship between any two items is reflected with an attention score. Pang \etal \cite{setrank} study the permutation-invariant property of the self-attention blocks in re-ranking. Feng \etal \cite{feng2021revisit} also investigate the permutation influence in re-ranking and generate candidate re-ranking permutations by beam search. Yet all of them overlook users' diversified interests towards the re-ranked lists.


 \subsection{Diversity}
In the context of search result diversification, explicit intent-aware diversity frameworks aim at promoting a hybrid of coverage over explicit aspects of a query and novelty. An early example of such kind of algorithm in information retrieval is the Maximum Marginal Relevance (MMR) re-ranking algorithm~\cite{carbonell1998use}. IA-Select \cite{agrawal2009diversifying} maximizes the probability that the average user finds at least one useful result within the top-$K$ results. PM-2 \cite{dang2012diversity} provides search results that best maintain the overall proportionality of documents belonging to different aspects. The intra-list similarity is calculated in \cite{ziegler2005improving} to diversify the topics in the list. xQuAD \cite{santos2010exploiting} is a probabilistic framework to balance relevance and novelty. However, result diversification in these information retrieval applications focuses on diversifying the search results over topic aspects and does not study users' personal diversified preferences towards the re-ranked lists. \wwadd{DPP NIPS'18}

% \url{https://zhuanlan.zhihu.com/p/72202739}
% calibrated recommendation
% Data-driven experiments on Huawei.
